BAXMC: a CEGAR approach to Max#SAT

Max#SAT is an important problem with multiple applications in security and program synthesis that is proven hard to solve. It is defined as: given a parameterized quantifier-free propositional formula compute parameters such that the number of models of the formula is maximal. As an extension, the formula can include an existential prefix. We propose a CEGAR-based algorithm and refinements thereof, based on either exact or approximate model counting, and prove its correctness in both cases. Our experiments show that this algorithm has much better effective complexity than the state of the art.

==> hardness.tex <==
We consider the following decision problem $\cproblem{DMax\#SAT}$, and generalizations thereof:
given a quantifier-free propositional formula $\phi(\VS{X},\VS{Y})$,
and a bound $B$, determine if there is $x$ such that $\countset{y \mid \phi(x, y)} \geq B$.
This is the decision version of the \MaxMC{} problem: finding $x$ and $B$ for maximal~$B$.

\begin{theorem}
  $\cproblem{DMax\#SAT}$ is $\existsclass{\PP}$-complete.
\end{theorem}

\begin{proof}
  It is in $\existsclass{\PP}$: it is well-known that taking $(\phi,B)$ as input and checking if
  $\countmodels{\phi} \geq B$ is in~$\PP$.

  Take a problem in $\existsclass{\PP}$.
  It can be reformulated as: take input $x$,
  choose nondeterministic bits $y$, construct a formula $\phi(x,y)$ with $N(x,y)$ variables, and check that
  $\Size{\{z \in \{0,1\}^{N(x,y)} \mid \phi(x,y)(z)\}} \geq 2^{N(x,y)-1}$.
  The condition $\phi(x,y)(z)$ can also be reformulated as $\exists z'~\psi(x,y,z,z')$ where $\psi$ simulates the action of the Turing machine that produces $\phi$ (if necessary by using temporary values in $z'$) then the semantics of the formula over~$z$.
  The result follows.
\end{proof}

Torán \cite[theorem 4.1 (ii)]{DBLP:journals/jacm/Toran91} showed a generalization of $\existsclass{\PP} =
\oracleclass{\NP}{\sharpP}$.
We give here a shorter proof of that result.

The following gadgets enable us to transform multiple equality tests over model counts
$\countmodels{\phi_1}=C_1 \land \dots \land \countmodels{\phi_m}=C_m$ into a single equality test over model counts.

\begin{definition}
  Let $\phi$ and $\psi$ be two quantifier-free propositional formulas with $n$ and $m$ variables
  respectively. Without loss of generality, we assume these variables to be $X_1,\dots,X_n$ and
  $X_{n+1},\dots,X_{n+m}$.
  Let $\Lambda_2^{m,n}(\phi,\psi)$ be the following formula over $m+n+2$ variables:
  \begin{multline*}
    \left(\phi(X_1,\dots,X_n) \land \neg{X_{n+1}} \land \dots \land \neg{X_{n+m+2}}\right) \\\lor
    \left(\psi(X_{n + 1},\dots,X_{n + m}) \land X_{n+m+1} \right)
  \end{multline*}
  $\size{\phi}$ denotes the size of a formula as the number of its Boolean operators, and $\countmodels{\phi}$ denotes the number of its models.
\end{definition}

\begin{lemma}
  $\size{\Lambda_2^{m,n}(\phi,\psi)} = \size{\phi} + \size{\psi} + m + 4$. Furthermore,
  $\countmodels{\phi}$ and $\countmodels{\psi}$ are respectively the remainder and quotient of
  $\countmodels{\Lambda_2^{m,n}(\phi,\psi)}$ by $2^{n+1}$.
\end{lemma}

% \begin{proof}
%   The size is obvious. For the number of models, each model of $F$ maps to one model of $\phi_2^{m,n}(F,G)$, and each model of $G$ to $2^{n+1}$ models of $\phi_2^{m,n}(F,G)$; these two disjoint sets make up the models of $\phi_2^{m,n}(F,G)$.
%   Quotient and remainder follow from $0 \leq \countmodels{G} \leq 2^n < 2^{n+1}$.
% \end{proof}

\begin{definition}
  Let $\phi_0,\dots$ be propositional formulas with $n$ variables.
  Let $\Lambda_1^n(\phi_0)=\phi_0$, $\Lambda_{k+1}^n(\phi_0,\dots,\phi_k) =
    \Lambda_2^{kn+2(k-1),n}(\Lambda_k^n(\phi_0,\dots,\phi_{k-1}), \phi_k)$.
\end{definition}

\begin{lemma}\label{lemma:count_base_decomposition}
  $\size{\Lambda_k^n(\phi_0,\dots,\phi_{k-1})} = \sum_i \size{\phi_i} + (k-1)(n+4)$.
  Furthermore, $\countmodels{\phi_i}$ is the digit of order $i$ of the
  decomposition of $\countmodels{\Lambda_k^{n}(\phi_0, \dots, \phi_{k-1})}$ in base $2^{n+1}$.
\end{lemma}

The following gadget will be used to add a number of models to an existing formula:
\begin{definition}
  Let $M^n_c(X_0,\dots,X_{n-1})$, where $0 \leq c \leq 2^n$, be the formula that specifies that $\sum_i 2^i X_i \leq c$.
\end{definition}

\begin{lemma}
  $\size{M^n_c}$ is linear in $n$ and $\countmodels{M^n_c}=c$.
\end{lemma}

The following gadget will be used to turn an equality test on the number of models of a formula into an inequality test:

\begin{definition}
  Let $\phi$ be a propositional formula over $n$ variables, and $0 \leq \Delta \leq 2{n-1}$.
  Let $\chi^n(\phi)$ be the formula over $2n+1$ variables
  \begin{multline*}
    \phi(X_1,\dots,X_n) \land \big(
    \left(\neg \phi(X_{n+1},\dots,X_{2n}) \land \neg X_{2n+1} \right) \\\lor
    \left(M^n_{2\Delta}(X_{n+1},\dots,X_{2n}) \land X_{2n+1}\right)\big)
  \end{multline*}
  Let $K^n_\Delta$ be the polynomial $K^n_\Delta(p) = p(2^n-p+2\Delta)$.
\end{definition}

\begin{lemma}\label{lem:model_count_eq_to_ineq}
  $\size{\chi^n(\phi)}$ has size linear in $\size{\phi}$, and
  $\countmodels{\chi^n(\phi)} = K^n_\Delta(\countmodels{\phi})$.
  Furthermore, $K^n_\Delta(\countmodels{\phi}) \geq K^n_\Delta(2^{n-1}+\Delta)$
  if and only if $\countmodels{\phi}=2^{n-1}+\Delta$.
\end{lemma}

\begin{theorem}
  $\existsclass{\PP} = \limitedoracleclass{\NP}{\PP}{1} = \oracleclass{\NP}{\PP} = \oracleclass{\NP}{\sharpP}$.
\end{theorem}

\begin{proof}
  Inclusions from left to right are trivial. We shall now prove that $\oracleclass{\NP}{\sharpP}$ is included in $\existsclass{\PP}$ by transforming a nondeterministic Turing machine $M$ deciding a problem $D(x)$ in time $P(\size{x})$ with a $\counting\SAT$ oracle into an equivalent decision procedure in $\existsclass{\PP}$.
  We proceed in steps:
  \begin{enumerate}
    \item $M$ calls the oracle at most $P(\size{x})$ times, over formulas of $P(\size{x})$ variables,
          and the outputs of each oracle call may be used for computing the inputs to further oracle
          calls. Instead, we transform the machine to non-deterministically choose all inputs $\phi_1,
            \dots, \phi_{P(\size{x})}$ and candidate outputs to the oracle calls ($\counting\SAT$), and
          then only at the end we verify that the candidate outputs $C_1,\dots,C_{P(\size{x})}$ match
          the real outputs $\countmodels{\phi_1},\dots,\countmodels{\phi_{P(\size{x})}}$ (we reject
          otherwise).
    \item We replace these calls by a single call to
          $\countmodels{\Lambda^{P(\size{x})}_{P(\size{x})}(\phi_1, \dots, \phi_{P(\size{x})})}$, and a
          single verification that the output $V$ of this call matches the candidate outputs
          $C_1,\dots,C_{P(\size{x})}$ according to the decomposition in \cref{lemma:count_base_decomposition}.
    \item We replace $\countmodels{\Lambda^{P(\size{x})}_{P(\size{x})}(\phi_1, \dots, \phi_{P(\size{x})})} = Y$ by a single call to $\counting\SAT$ and an inequality test as follows.
          Let $n$ be the number of variables of $\Lambda^{P(\size{x})}_{P(\size{x})}(\phi_1, \dots,
          \phi_{P(\size{x})})$:
          \begin{itemize}
            \item If $Y \geq 2^{n-1}$, then write $Y = 2^{n-1} + \Delta$.
                  Then we replace the equality test by an inequality test
                  $\countmodels{\chi^n(\Lambda^{P(\size{x})}_{P(\size{x})}(\phi_1, \dots, \phi_{P(\size{x})}))} \geq K^n_\Delta$, according to \cref{lem:model_count_eq_to_ineq}.
            \item If $Y < 2^{n-1}$, then write $Y = 2^{n-1} - \Delta$.
                  Then we replace the equality test by an inequality test
                  $\countmodels{\chi^n(\neg \Lambda^{P(\size{x})}_{P(\size{x})}(\phi_1, \dots, \phi_{P(\size{x})}))} \geq K^n_\Delta$, according to \cref{lem:model_count_eq_to_ineq}.
          \end{itemize}
    \item We have thus reduced the procedure to the nondeterministic (possibly failing) construction of a pair $(G,B)$ followed by a test $\countmodels{G} \geq B$.
          This test is well-known to be complete for~$\PP$.
  \end{enumerate}
\end{proof}

\begin{corollary}
  $\cproblem{DMax\#SAT}$ is hard for the polynomial hierarchy.
\end{corollary}

\begin{proof}
  Obviously, $\oracleclass{\Pclass}{\sharpP} \subseteq \oracleclass{\NP}{\sharpP}$, and the former class is hard for the polynomial hierarchy by Toda's theorem.
\end{proof}

\begin{remark}
  The above results consider quantifier-free propositional formulas over a number of free variables.
  In fact, we can use arbitrary predicates with a certain number of free variables: for instance,
  take inputs $X_1,\dots,X_n$, and return \emph{true} or \emph{false} depending on whether a certain polynomial-time nondeterministic Turing machine parameterized by $X_1,\dots,X_n$ has an accepting run or not.
  Hence, we could consider predicates of the form $\exists Z_1,\dots,Z_p~ \phi(X_1,\dots,X_n, Z_1,\dots,Z_p)$.
  We then obtain the result
  $\existsclass{\majorityclass{\NP}} = \oracleclass{\NP}{\counting{\NP}}$.

  Going with classes of predicates arbitrarily high in the counting hierarchy, we
  obtain \cite[theorem 4.1 (ii)]{DBLP:journals/jacm/Toran91}:

  \begin{theorem}
    For any class $K$ in the counting hierarchy,
    $\existsclass{\majorityclass{K}} = \limitedoracleclass{\NP}{\majorityclass{K}}{1} = \oracleclass{\NP}{\majorityclass{K}} = \oracleclass{\NP}{\counting{K}}$.
  \end{theorem}
\end{remark}

